Polygones fondamentaux d'une courbe modulaire

A few pages in Siegel describe how, starting with a fundamental polygon for a compact Riemann surface, one can construct a symplectic basis of its homology. This note retells that construction, specializing to the case where the surface is associated to a congruence subgroup $\Gamma$ of $SL_2(Z)$. One then obtains by classical procedures a generating system for $\Gamma$ with a minimal number of hyperbolic elements and a presentation of the $Z[\Gamma]$-module $Z[P^1(Q)]_0$.

==> fareydraw/0_15.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{4}}}{\underparen{}}1


==> fareydraw/0_16.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{3}{8}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{5}}}{\underparen{}}1


==> fareydraw/0_17.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{\underset{\circ}{\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{3}
\underset{\underset{\circ}{\aaa_{4}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{5}}}{\underparen{}}1


==> fareydraw/0_18.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{6}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{2}{9}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{5}{9}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{4}{7}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{7}{12}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{7}}}{\underparen{}}1


==> fareydraw/0_19.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{3}
\underset{\underset{\bullet}{\aaa_{4}}}{\underparen{}}\frac{1}{2}
\underset{\underset{\bullet}{\aaa_{5}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{3}}}{\underparen{}}1


==> fareydraw/0_21.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{\underset{\bullet}{\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{2}{7}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{3}{7}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{5}{7}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{3}{4}
\underset{\underset{\bullet}{\aaa_{7}}}{\underparen{}}1


==> fareydraw/0_22.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{3}{11}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{2}{7}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{4}{11}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{3}{8}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{7}}}{\underparen{}}1


==> fareydraw/0_23.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{5}}}{\underparen{}}1


==> fareydraw/0_24.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{7}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{6}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{3}{8}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{5}{13}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{8}}}{\underparen{}}\frac{5}{12}
\underset{ {\aaa^*_{8}}}{\underparen{}}\frac{3}{7}
\underset{ {\aaa_{9}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{9}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{5}{8}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{4}}}{\underparen{}}1


==> fareydraw/0_25.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{1}{4}
\underset{\underset{\circ}{\aaa_{3}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{2}{3}
\underset{\underset{\circ}{\aaa_{6}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{4}{5}
\underset{ {\aaa^*_{7}}}{\underparen{}}1


==> fareydraw/0_26.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{\underset{\circ}{\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{8}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{5}{13}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa_{8}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{8}{13}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{5}{8}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{8}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{4}{5}
\underset{\underset{\circ}{\aaa_{9}}}{\underparen{}}1


==> fareydraw/0_27.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{2}{9}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{7}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{4}{9}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{5}}}{\underparen{}}1


==> fareydraw/0_28.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{3}{14}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{2}{9}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{2}{7}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{3}{7}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{4}{7}
\underset{ {\aaa_{8}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa_{9}}}{\underparen{}}\frac{5}{8}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{8}}}{\underparen{}}\frac{5}{7}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{9}}}{\underparen{}}1


==> fareydraw/0_29.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{2}{5}
\underset{\underset{\circ}{\aaa_{6}}}{\underparen{}}\frac{1}{2}
\underset{\underset{\circ}{\aaa_{7}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{4}{5}
\underset{ {\aaa^*_{3}}}{\underparen{}}1


==> fareydraw/0_31.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{\underset{\bullet}{\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{4}
\underset{\underset{\bullet}{\aaa_{4}}}{\underparen{}}\frac{2}{7}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{5}}}{\underparen{}}1


==> fareydraw/0_35.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{6}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{3}{11}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{2}{7}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{3}{7}
\underset{ {\aaa_{8}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{4}{7}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{5}{8}
\underset{ {\aaa_{9}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{8}}}{\underparen{}}\frac{5}{7}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{9}}}{\underparen{}}1


==> fareydraw/1_16.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{3}{8}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa^*_{5}}}{\underparen{}}1


==> fareydraw/1_17.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{\underset{\circ}{\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{3}{8}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{11}{29}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{8}{21}
\underset{\underset{\circ}{\aaa_{5}}}{\underparen{}}1


==> fareydraw/1_18.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{6}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{2}{9}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{3}{13}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{6}{23}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{4}{7}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{7}{12}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{2}{3}
\underset{ {\aaa^*_{7}}}{\underparen{}}1


==> fareydraw/1_19.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{8}{23}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{7}{20}
\underset{\underset{\bullet}{\aaa_{4}}}{\underparen{}}\frac{4}{11}
\underset{\underset{\bullet}{\aaa_{5}}}{\underparen{}}1


==> fareydraw/1_21.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{\underset{\bullet}{\aaa_{2}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{7}{27}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{48}{185}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{89}{343}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{219}{844}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{13}{50}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{3}{10}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{7}{16}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{3}{4}
\underset{\underset{\bullet}{\aaa_{7}}}{\underparen{}}1


==> fareydraw/1_22.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{18}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{11}{197}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{15}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{6}{23}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{94}{355}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{431}{1627}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{11}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{409}{1453}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{20}{71}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{5}{17}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{8}{23}
\underset{ {\aaa^*_{7}}}{\underparen{}}1


==> fareydraw/1_23.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{10}{49}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{29}{142}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{19}{93}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{3}{14}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{10}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{7}{19}
\underset{ {\aaa^*_{5}}}{\underparen{}}1


==> fareydraw/1_24.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{12}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{1}{11}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{10}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{5}{49}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{9}{88}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{22}{215}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{4}{39}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{42}{409}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{7}{68}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{105}{1019}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{3}{29}
\underset{ {\aaa_{8}}}{\underparen{}}\frac{1}{7}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{29}{191}
\underset{ {\aaa^*_{8}}}{\underparen{}}\frac{9}{59}
\underset{ {\aaa_{9}}}{\underparen{}}\frac{1}{6}
\underset{ {\aaa^*_{9}}}{\underparen{}}1


==> fareydraw/1_25.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{1}{4}
\underset{\underset{\circ}{\aaa_{3}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{1}{2}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{5}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{2}{3}
\underset{\underset{\circ}{\aaa_{6}}}{\underparen{}}\frac{3}{4}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{4}{5}
\underset{ {\aaa^*_{7}}}{\underparen{}}1


==> fareydraw/1_26.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{\underset{\circ}{\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{8}{39}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{15}{73}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{7}{34}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{76}{369}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{14}{67}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{9}{35}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{115}{439}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{22}{83}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{13}{49}
\underset{ {\aaa_{8}}}{\underparen{}}\frac{1}{3}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{2}{5}
\underset{ {\aaa^*_{8}}}{\underparen{}}\frac{4}{5}
\underset{\underset{\circ}{\aaa_{9}}}{\underparen{}}1


==> fareydraw/1_27.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{6}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{3}{17}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{2}{11}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{7}{34}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{48}{233}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{13}{63}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{17}{82}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{5}{24}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{13}{62}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{2}{9}
\underset{ {\aaa^*_{7}}}{\underparen{}}1


==> fareydraw/1_28.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{24}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{7}{167}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{5}{119}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{33}{785}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{1}{19}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{5}{33}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{151}{965}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{193}{1233}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{1}{6}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{332}{1917}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{3}{17}
\underset{ {\aaa_{8}}}{\underparen{}}\frac{8}{39}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{149}{713}
\underset{ {\aaa^*_{8}}}{\underparen{}}\frac{32}{153}
\underset{ {\aaa_{9}}}{\underparen{}}\frac{3}{14}
\underset{ {\aaa^*_{9}}}{\underparen{}}1


==> fareydraw/1_29.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{16}{63}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{15}{59}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{3}{11}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{8}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{21}{52}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{24}{59}
\underset{\underset{\circ}{\aaa_{6}}}{\underparen{}}\frac{7}{17}
\underset{\underset{\circ}{\aaa_{7}}}{\underparen{}}1


==> fareydraw/1_31.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{\underset{\bullet}{\aaa_{2}}}{\underparen{}}\frac{1}{5}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{1}{4}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{4}{15}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{55}{206}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{51}{191}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{34}{127}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{41}{153}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{73}{272}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{18}{67}
\underset{\underset{\bullet}{\aaa_{7}}}{\underparen{}}1


==> fareydraw/1_35.tex <==
1
\underset{ {\aaa_{1}}}{\underparen{}}\infty
\underset{ {\aaa^*_{1}}}{\underparen{}}0
\underset{ {\aaa_{2}}}{\underparen{}}\frac{1}{7}
\underset{ {\aaa^*_{2}}}{\underparen{}}\frac{5}{34}
\underset{ {\aaa_{3}}}{\underparen{}}\frac{9}{61}
\underset{ {\aaa_{4}}}{\underparen{}}\frac{4}{27}
\underset{ {\aaa^*_{3}}}{\underparen{}}\frac{67}{452}
\underset{ {\aaa^*_{4}}}{\underparen{}}\frac{197}{1329}
\underset{ {\aaa_{5}}}{\underparen{}}\frac{3}{20}
\underset{ {\aaa^*_{5}}}{\underparen{}}\frac{790}{5251}
\underset{ {\aaa_{6}}}{\underparen{}}\frac{229}{1521}
\underset{ {\aaa_{7}}}{\underparen{}}\frac{55}{356}
\underset{ {\aaa^*_{6}}}{\underparen{}}\frac{214}{1369}
\underset{ {\aaa^*_{7}}}{\underparen{}}\frac{1085}{6931}
\underset{ {\aaa_{8}}}{\underparen{}}\frac{8}{51}
\underset{ {\aaa_{9}}}{\underparen{}}\frac{5}{27}
\underset{ {\aaa^*_{8}}}{\underparen{}}\frac{14}{53}
\underset{ {\aaa^*_{9}}}{\underparen{}}1


==> fareydraw/cercle0_10.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{45};
\draw \unarc{3}{$\aaa_{2}$}{45};
\draw \cell{3}{45};
\draw \link {4}{$\aaa_{3}$}{7}{$\aaa^*_{3}$}{45};
\draw \link {5}{$\aaa_{4}$}{6}{$\aaa^*_{4}$}{45};
\draw \unarc{8}{$\aaa_{5}$}{45};
\draw \cell{8}{45};



==> fareydraw/cercle0_12.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{36};
\draw \slink {5}{$\aaa_{3}$}{10}{$\aaa^*_{3}$}{36};
\draw \link {6}{$\aaa_{4}$}{9}{$\aaa^*_{4}$}{36};
\draw \link {7}{$\aaa_{5}$}{8}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle0_14.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{9}{$\aaa^*_{2}$}{36};
\draw \link {4}{$\aaa_{3}$}{8}{$\aaa^*_{3}$}{36};
\draw \link {5}{$\aaa_{4}$}{7}{$\aaa^*_{4}$}{36};
\draw \link {6}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle0_15.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{7}{$\aaa^*_{2}$}{36};
\draw \link {4}{$\aaa_{3}$}{8}{$\aaa^*_{3}$}{36};
\draw \slink {5}{$\aaa_{4}$}{10}{$\aaa^*_{4}$}{36};
\draw \link {6}{$\aaa_{5}$}{9}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle0_16.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{36};
\draw \link {5}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{36};
\draw \link {7}{$\aaa_{4}$}{8}{$\aaa^*_{4}$}{36};
\draw \link {9}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle0_17.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{45};
\draw \unarc{3}{$\aaa_{2}$}{45};
\draw \cell{3}{45};
\draw \link {4}{$\aaa_{3}$}{7}{$\aaa^*_{3}$}{45};
\draw \unarc{5}{$\aaa_{4}$}{45};
\draw \cell{5}{45};
\draw \link {6}{$\aaa_{5}$}{8}{$\aaa^*_{5}$}{45};



==> fareydraw/cercle0_18.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{180/7};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{180/7};
\draw \link {5}{$\aaa_{3}$}{10}{$\aaa^*_{3}$}{180/7};
\draw \link {6}{$\aaa_{4}$}{9}{$\aaa^*_{4}$}{180/7};
\draw \link {7}{$\aaa_{5}$}{8}{$\aaa^*_{5}$}{180/7};
\draw \link {11}{$\aaa_{6}$}{12}{$\aaa^*_{6}$}{180/7};
\draw \link {13}{$\aaa_{7}$}{14}{$\aaa^*_{7}$}{180/7};



==> fareydraw/cercle0_19.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{45};
\draw \slink {3}{$\aaa_{2}$}{7}{$\aaa^*_{2}$}{45};
\draw \slink {4}{$\aaa_{3}$}{8}{$\aaa^*_{3}$}{45};
\draw \unarc{5}{$\aaa_{4}$}{45};
\draw \cell{5}{45};
\fill \cell{5}{45};
\draw \unarc{6}{$\aaa_{5}$}{45};
\draw \cell{6}{45};
\fill \cell{6}{45};



==> fareydraw/cercle0_22.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{180/7};
\draw \link {3}{$\aaa_{2}$}{11}{$\aaa^*_{2}$}{180/7};
\draw \link {4}{$\aaa_{3}$}{8}{$\aaa^*_{3}$}{180/7};
\draw \link {5}{$\aaa_{4}$}{7}{$\aaa^*_{4}$}{180/7};
\draw \link {6}{$\aaa_{5}$}{12}{$\aaa^*_{5}$}{180/7};
\draw \link {9}{$\aaa_{6}$}{13}{$\aaa^*_{6}$}{180/7};
\draw \link {10}{$\aaa_{7}$}{14}{$\aaa^*_{7}$}{180/7};



==> fareydraw/cercle0_23.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{5}{$\aaa^*_{2}$}{36};
\draw \link {4}{$\aaa_{3}$}{7}{$\aaa^*_{3}$}{36};
\draw \link {6}{$\aaa_{4}$}{9}{$\aaa^*_{4}$}{36};
\draw \link {8}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle0_25.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{30};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{30};
\draw \unarc{5}{$\aaa_{3}$}{30};
\draw \cell{5}{30};
\draw \link {6}{$\aaa_{4}$}{7}{$\aaa^*_{4}$}{30};
\draw \link {8}{$\aaa_{5}$}{9}{$\aaa^*_{5}$}{30};
\draw \unarc{10}{$\aaa_{6}$}{30};
\draw \cell{10}{30};
\draw \link {11}{$\aaa_{7}$}{12}{$\aaa^*_{7}$}{30};



==> fareydraw/cercle0_27.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{180/7};
\draw \link {3}{$\aaa_{2}$}{11}{$\aaa^*_{2}$}{180/7};
\draw \link {4}{$\aaa_{3}$}{5}{$\aaa^*_{3}$}{180/7};
\draw \link {6}{$\aaa_{4}$}{7}{$\aaa^*_{4}$}{180/7};
\draw \link {8}{$\aaa_{5}$}{14}{$\aaa^*_{5}$}{180/7};
\draw \link {9}{$\aaa_{6}$}{10}{$\aaa^*_{6}$}{180/7};
\draw \link {12}{$\aaa_{7}$}{13}{$\aaa^*_{7}$}{180/7};



==> fareydraw/cercle0_29.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{30};
\draw \link {3}{$\aaa_{2}$}{11}{$\aaa^*_{2}$}{30};
\draw \link {4}{$\aaa_{3}$}{12}{$\aaa^*_{3}$}{30};
\draw \link {5}{$\aaa_{4}$}{9}{$\aaa^*_{4}$}{30};
\draw \link {6}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{30};
\draw \unarc{7}{$\aaa_{6}$}{30};
\draw \cell{7}{30};
\draw \unarc{8}{$\aaa_{7}$}{30};
\draw \cell{8}{30};



==> fareydraw/cercle1_10.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{45};
\draw \unarc{3}{$\aaa_{2}$}{45};
\draw \cell{3}{45};
\draw \link {4}{$\aaa_{3}$}{5}{$\aaa^*_{3}$}{45};
\draw \link {6}{$\aaa_{4}$}{7}{$\aaa^*_{4}$}{45};
\draw \unarc{8}{$\aaa_{5}$}{45};
\draw \cell{8}{45};



==> fareydraw/cercle1_12.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{36};
\draw \link {5}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{36};
\draw \link {7}{$\aaa_{4}$}{8}{$\aaa^*_{4}$}{36};
\draw \link {9}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle1_14.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{36};
\draw \link {5}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{36};
\draw \link {7}{$\aaa_{4}$}{9}{$\aaa^*_{4}$}{36};
\draw \link {8}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle1_15.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{36};
\draw \link {5}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{36};
\draw \link {7}{$\aaa_{4}$}{9}{$\aaa^*_{4}$}{36};
\draw \link {8}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle1_16.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{36};
\draw \link {5}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{36};
\draw \link {7}{$\aaa_{4}$}{8}{$\aaa^*_{4}$}{36};
\draw \link {9}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle1_17.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{45};
\draw \unarc{3}{$\aaa_{2}$}{45};
\draw \cell{3}{45};
\draw \link {4}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{45};
\draw \link {5}{$\aaa_{4}$}{7}{$\aaa^*_{4}$}{45};
\draw \unarc{8}{$\aaa_{5}$}{45};
\draw \cell{8}{45};



==> fareydraw/cercle1_18.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{180/7};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{180/7};
\draw \link {5}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{180/7};
\draw \link {7}{$\aaa_{4}$}{8}{$\aaa^*_{4}$}{180/7};
\draw \link {9}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{180/7};
\draw \link {11}{$\aaa_{6}$}{12}{$\aaa^*_{6}$}{180/7};
\draw \link {13}{$\aaa_{7}$}{14}{$\aaa^*_{7}$}{180/7};



==> fareydraw/cercle1_19.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{45};
\draw \link {3}{$\aaa_{2}$}{5}{$\aaa^*_{2}$}{45};
\draw \link {4}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{45};
\draw \unarc{7}{$\aaa_{4}$}{45};
\draw \cell{7}{45};
\fill \cell{7}{45};
\draw \unarc{8}{$\aaa_{5}$}{45};
\draw \cell{8}{45};
\fill \cell{8}{45};



==> fareydraw/cercle1_22.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{180/7};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{180/7};
\draw \link {5}{$\aaa_{3}$}{7}{$\aaa^*_{3}$}{180/7};
\draw \link {6}{$\aaa_{4}$}{8}{$\aaa^*_{4}$}{180/7};
\draw \link {9}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{180/7};
\draw \link {11}{$\aaa_{6}$}{13}{$\aaa^*_{6}$}{180/7};
\draw \link {12}{$\aaa_{7}$}{14}{$\aaa^*_{7}$}{180/7};



==> fareydraw/cercle1_23.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{36};
\draw \link {3}{$\aaa_{2}$}{5}{$\aaa^*_{2}$}{36};
\draw \link {4}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{36};
\draw \link {7}{$\aaa_{4}$}{9}{$\aaa^*_{4}$}{36};
\draw \link {8}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{36};



==> fareydraw/cercle1_25.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{30};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{30};
\draw \unarc{5}{$\aaa_{3}$}{30};
\draw \cell{5}{30};
\draw \link {6}{$\aaa_{4}$}{7}{$\aaa^*_{4}$}{30};
\draw \link {8}{$\aaa_{5}$}{9}{$\aaa^*_{5}$}{30};
\draw \unarc{10}{$\aaa_{6}$}{30};
\draw \cell{10}{30};
\draw \link {11}{$\aaa_{7}$}{12}{$\aaa^*_{7}$}{30};



==> fareydraw/cercle1_27.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{180/7};
\draw \link {3}{$\aaa_{2}$}{4}{$\aaa^*_{2}$}{180/7};
\draw \link {5}{$\aaa_{3}$}{7}{$\aaa^*_{3}$}{180/7};
\draw \link {6}{$\aaa_{4}$}{8}{$\aaa^*_{4}$}{180/7};
\draw \link {9}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{180/7};
\draw \link {11}{$\aaa_{6}$}{12}{$\aaa^*_{6}$}{180/7};
\draw \link {13}{$\aaa_{7}$}{14}{$\aaa^*_{7}$}{180/7};



==> fareydraw/cercle1_29.tex <==
\draw \link {1}{$\aaa_{1}$}{2}{$\aaa^*_{1}$}{30};
\draw \link {3}{$\aaa_{2}$}{5}{$\aaa^*_{2}$}{30};
\draw \link {4}{$\aaa_{3}$}{6}{$\aaa^*_{3}$}{30};
\draw \link {7}{$\aaa_{4}$}{9}{$\aaa^*_{4}$}{30};
\draw \link {8}{$\aaa_{5}$}{10}{$\aaa^*_{5}$}{30};
\draw \unarc{11}{$\aaa_{6}$}{30};
\draw \cell{11}{30};
\draw \unarc{12}{$\aaa_{7}$}{30};
\draw \cell{12}{30};



==> polygondraw/0_12.tex <==

\begin{tikzpicture}[scale=10]
\scriptsize
\draw (0,0.50000000)--(0,0) node [very near start, right] {$\aaa_1^*$} node [below] {$0$}node (start) {} arc (180:0:0.083333333)  node [midway, above] {$\aaa_{2}$} node [below]{$\frac{1}{6}$} 
node (start) {} arc (180:0:0.016666667)  node [midway, above] {$\aaa^*_{2}$} node [below]{$\frac{1}{5}$} 
node (start) {} arc (180:0:0.025000000)  node [midway, above] {$\aaa_{3}$} node [below]{$\frac{1}{4}$} 
node (start) {} arc (180:0:0.041666667)  node [midway, above] {$\aaa_{4}$} node [below]{$\frac{1}{3}$} 
node (start) {} arc (180:0:0.083333333)  node [midway, above] {$\aaa_{5}$} node [below]{$\frac{1}{2}$} 
node (start) {} arc (180:0:0.083333333)  node [midway, above] {$\aaa^*_{5}$} node [below]{$\frac{2}{3}$} 
node (start) {} arc (180:0:0.041666667)  node [midway, above] {$\aaa^*_{4}$} node [below]{$\frac{3}{4}$} 
node (start) {} arc (180:0:1/8)  node [midway, above] {$\aaa^*_{3}$} node [below] {$1$} -- (1,0.50000000) node [very near end, left] {$\aaa_1$};
    \end{tikzpicture}


==> polygondraw/2_12.tex <==

\begin{tikzpicture}[scale=10]
\scriptsize
\draw (0,0.50000000)--(0,0) node [very near start, right] {$\aaa_1^*$} node [below] {$0$}node (start) {} arc (180:0:0.083333333)  node [midway, above] {$\aaa_{2}$} node [below]{$\frac{1}{6}$} 
node (start) {} arc (180:0:0.016666667)  node [midway, above] {$\aaa^*_{2}$} node [below]{$\frac{1}{5}$} 
node (start) {} arc (180:0:0.025000000)  node [midway, above] {$\aaa_{3}$} node [below]{$\frac{1}{4}$} 
node (start) {} arc (180:0:0.017857143)  node [midway, above] {$\aaa^*_{3}$} node [below]{$\frac{2}{7}$} 
node (start) {} arc (180:0:0.023809524)  node [midway, above] {$\aaa_{4}$} node [below]{$\frac{1}{3}$} 
node (start) {} arc (180:0:0.033333333)  node [midway, above] {$\aaa^*_{4}$} node [below]{$\frac{2}{5}$} 
node (start) {} arc (180:0:0.050000000)  node [midway, above] {$\aaa_{5}$} node [below]{$\frac{1}{2}$} 
node (start) {} arc (180:0:1/4)  node [midway, above] {$\aaa^*_{5}$} node [below] {$1$} -- (1,0.50000000) node [very near end, left] {$\aaa_1$};
    \end{tikzpicture}


==> polygondraw/2_13.tex <==

\begin{tikzpicture}[scale=10]
\scriptsize
\draw (0,0.50000000)--(0,0) node [very near start, right] {$\aaa_1^*$} node [below] {$0$}node (start) {} arc (180:0:0.16666667)  node [midway, above] {$\aaa_{2}$} node [below]{$\frac{1}{3}$};
 \draw (start) arc (180:28:0.14285714) node {$\bullet$} arc (88:0:0.066666667) 
node (start) {} arc (180:0:0.083333333)  node [midway, above] {$\aaa_{3}$} node [below]{$\frac{1}{2}$} node (start) {} (5/13,1/13) node {$\circ$};
 \draw (start) node{} 
node (start) {} arc (180:0:0.083333333)  node [midway, above] {$\aaa_{4}$} node [below]{$\frac{2}{3}$} node (start) {} (8/13,1/13) node {$\circ$};
 \draw (start) node{} 
node (start) {} arc (180:0:1/6)  node [midway, above] {$\aaa_{5}$};
 \draw (start) arc (180:92:0.066666667) node {$\bullet$} arc (152:0:0.14285714) node [below] {$1$} -- (1,0.50000000) node [very near end, left] {$\aaa_1$};
    \end{tikzpicture}

